Improving Gaussian Splatting with Localized Points Management

Point management is critical for optimizing 3D Gaussian Splatting models, as point initiation (e.g., via structure from motion) is often distributionally inappropriate. Typically, Adaptive Density Control (ADC) algorithm is adopted, leveraging view-averaged gradient magnitude thresholding for point densification, opacity thresholding for pruning, and regular all-points opacity reset. We reveal that this strategy is limited in tackling intricate/special image regions (e.g., transparent) due to inability of identifying all 3D zones requiring point densification, and lacking an appropriate mechanism to handle ill-conditioned points with negative impacts (e.g., occlusion due to false high opacity). To address these limitations, we propose a Localized Point Management (LPM) strategy, capable of identifying those error-contributing zones in greatest need for both point addition and geometry calibration. Zone identification is achieved by leveraging the underlying multiview geometry constraints, subject to image rendering errors. We apply point densification in the identified zones and then reset the opacity of the points in front of these regions, creating a new opportunity to correct poorly conditioned points. Serving as a versatile plugin, LPM can be seamlessly integrated into existing static 3D and dynamic 4D Gaussian Splatting models with minimal additional cost. Experimental evaluations validate the efficacy of our LPM in boosting a variety of existing 3D/4D models both quantitatively and qualitatively. Notably, LPM improves both static 3DGS and dynamic SpaceTimeGS to achieve state-of-the-art rendering quality while retaining real-time speeds, excelling on challenging datasets such as Tanks & Temples and the Neural 3D Video dataset.

==> tables/ab_error.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{PlayRoom} & \multicolumn{3}{c}{Truck} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\multirow{1}{*}{\centering Method} & PSNR & LPIPS & SSIM & PSNR & LPIPS & SSIM \\
\midrule
{L1 } & 30.21 & 0.241 & 0.910 & 25.61 & 0.154 &0.883 \\
% wo/ add new gaussians & 32.30 & 0.108 & 1398367 & 34.23 & 0.032 & 271387 \\
{L2} & - & -& - &- & - & - \\
{SSIM}& - & -& - &- & - & -  \\
\bottomrule
\end{tabular}
\caption{Performance comparison for different way to generate the error map.}
\label{tab:module_ab}
\end{table}


==> tables/db_tanks.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Method} & \multicolumn{3}{c}{\textbf{Tanks\&Temples}} & \multicolumn{3}{c}{\textbf{Deep Blending}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS \\
\midrule
Plenoxels     & 21.08  & 0.719 &  0.379 & 23.06 & 0.795 &  0.510 \\
INGP-Big    & 21.92 & 0.745 & 0.305 & 24.96 & 0.817 & 0.390 \\
Mip-NeRF 360   & 22.22 & 0.759 &0.257 & 29.40 & 0.901 & 0.245 \\
3DGS         & 29.4  &0.903 & 0.243 & 23.7 & 0.846&  0.179 \\
3DGS*         & 29.55 & 0.904 & 0.245 & 23.66 & 0.849 & 0.177 \\
3DGS + \textbf{\shortname{} }   & \textbf{29.76} & 0.908& 0.241& \textbf{23.81} & 0.85 & 0.182 \\
\bottomrule
\end{tabular}
\caption{Comparison of various methods across different scenes on the Mip-NeRF 360 dataset}
\label{tab:results}
\end{table}


==> tables/fsgs_lpm.tex <==
% \begin{table*}[ht]
% \setlength\tabcolsep{4pt} 
% \centering

% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \textbf{Reset Inter.} & \multicolumn{3}{c}{\textbf{Indoor}} & \multicolumn{3}{c}{\textbf{Outdoor}}\\ 
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
% & PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS  \\
% \midrule
% 100       &  31.035 & 0.926 & 0.184 & 24.83 & 0.7344 & 0.2438 \\
% 200   & 29.85 & 0.90 & 0.190 & 25.12 & 0.7412 & 0.2235\\
% \bottomrule
% \end{tabular}
% \caption{Comparison.}
% \label{tab:lpm_reset_ini}
% \end{table*}

\begin{table}[ht]
\setlength\tabcolsep{3pt} 
\centering
\scriptsize
\vspace{-6pt}
\begin{tabular}{lccc}
\toprule
Method & PSNR & SSIM & LPIPS  \\
\midrule
FSGS  &  22.13 & 0.600 & 0.389 \\
FSGS+LPM  & 22.42  & 0.646 & 0.351   \\
\bottomrule
\end{tabular}

\caption{LPM in sparse view setting (Mip-NeRF 360, 24 views).}
\label{tab:sp_lpm}
\vspace{-8pt}
\end{table}


==> tables/lpm_reset_ini.tex <==
\begin{table}[ht]
\setlength\tabcolsep{3pt} 
\centering
\scriptsize

\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Reset Inter.} & \multicolumn{3}{c}{\textbf{Indoor}} & \multicolumn{3}{c}{\textbf{Outdoor}}\\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
& PSNR & SSIM & LPIPS & PSNR & SSIM & LPIPS  \\
\midrule
100  &  31.03 & 0.926 & 0.184 & 24.83 & 0.734 & 0.243 \\
200  & 29.85  & 0.900  & 0.190  & 25.12 & 0.741 & 0.223 \\
\bottomrule
\end{tabular}
\caption{Ablation of reset intervals.}
\vspace{-5pt}
\label{tab:lpm_reset_ini}
\end{table}

